Meet Your Favorite Character: Open-domain Chatbot Mimicking Fictional Characters with only a Few Utterances

In this paper, we consider mimicking fictional characters as a promising direction for building engaging conversation models. To this end, we present a new practical task where only a few utterances of each fictional character are available to generate responses mimicking them. Furthermore, we propose a new method named Pseudo Dialog Prompting (PDP) that generates responses by leveraging the power of large-scale language models with prompts containing the target character's utterances. To better reflect the style of the character, PDP builds the prompts in the form of dialog that includes the character's utterances as dialog history. Since only utterances of the characters are available in the proposed task, PDP matches each utterance with an appropriate pseudo-context from a predefined set of context candidates using a retrieval model. Through human and automatic evaluation, we show that PDP generates responses that better reflect the style of fictional characters than baseline methods.

==> Sections/AuthorResponse.tex <==
\clearpage
\newpage
\section*{Author Response for Paper \#1234 (ARR 2021 November)}
We sincerely thank all the reviewers for their constructive feedback. 
We are especially encouraged that all the reviewers and Area Chair (\AC) find our problem setting is interesting, and  [\Rone,\Rthr] mention this problem is also challenging. 
Moreover, [\AC,\Rone,\Rfour] think our proposed method is simple and straightforward, and [\Rthr,\Rfour] find the method is interesting.
We are also pleased that [\AC,\Rfour] agree that we provide detailed experiments and analysis.
We correct the issues raised by the reviewers and attach the revised version with highlighted modifications.
\section*{Recap}
\textbf{What is our goal?} 
(1) Mimicking an arbitrary character where only a few utterances of the fictional character are available to generate the identifiable responses.
(2) To address the described task, we suggest a simple yet effective method which builds a dialog format prompt by matching pseudo-contexts with given few utterances.
\newline
\noindent \textbf{What is \textit{not} our goal?}
(1) We do not aim the task where large amount of utterances for the fictional character are available.
(2) Our focus is not proposing a good context selection strategy.

\section*{Responses}
\noindent \textbf{
[\Rone, \Rthr: Need to compare with style transfer / stylized dialogue generation literatures]
}

Most of the style transfer and stylized dialogue generation literature we have checked (including all the papers that reviewer [\Rone] and [\Rthr] mentioned) has a major difference with our problem setting such that all the works require additional training using a large number of parallel or unparallel target-style sentences (at least 10K in all experiments).
In contrast, our problem setting focuses on the case when there are only a few utterances of a mimicking character.
Therefore, we did not consider the methods requiring additional training with numerous style-labeled utterances.
Instead, we incorporate TextSETTR as our baseline representing a style-transfer based model that can be trained without style-labeled texts, and inference can be performed only using few-shot examples of a target style.
As this criterion of selecting the baseline methods are not extensively discussed in the original version of the paper, we included additional details on the criterion in the paper and added Related Work section in the Appendix to clarify the difference between existing style transfer / stylized dialogue generation literatures and our problem setting.

\noindent \textbf{
[\Rone: How is this work addresses open-domain conversation]
}

Our work addresses the challenges of mimicking characters with only a few utterances in the open-domain conversation, which is the main point of the work.
To be more precise, our method utilizes the utterances from large open-domain conversation datasets (A union of Blended Skill Talk, ConvAI2, Empathetic Dialogues, and Wizard of Wikipedia) to construct a pseudo-context, covering a diverse range of topics and situations.
We also want to note that BlenderBot\footnote{Recipes for building an open-domain chatbot, EACL 2021}, which is one of the most popular open-domain conversation model, also uses a same union of dataset as our setting.
Moreover, our experiments are done with DailyDialog dataset, which is also a well-known open-domain conversation set.
% Furthermore, pseudo context-response pairs generated by PDP only indirectly influences the model by being utilized as a prompt of the language model and do not replace the original context of the dialogue.
% Therefore, our model is not bound to converse only about the context/topic in the training dataset.
Various response examples illustrated in Table 2, Table 12, Figure 3, Figure 4 sufficiently demonstrate that our model can converse about diverse topics.

\noindent \textbf{
[\Rone: Need to compare with complex context selection strategy such as DialogBERT]
}

We totally agree with the suggestion that utilizing more complex context retrieval methods is a promising way to improve the performance of PDP methods.
However, we want to clarify that the goal of this work is not proposing a good context selection strategy.
Instead, our goal is to verify our main argument that "constructing an LM prompt as a dialog format utilizing pseudo context-response pairs is beneficial for mimicking fictional characters".
Thus, we think using a complex retrieval method is not a mandatory baseline for our experiment.
% In addition, DialogBERT mainly focuses on modeling multi-turn contexts using hierarchical encoders.
% Since we only use single-turn context candidates in our experiments, utilizing DialogBERT might not be highly beneficial for our context retrieval.
Yet, we agree that using complex context retrieval methods is a promising way to improve the PDP method, so it must be an interesting following work.

\noindent \textbf{
[\Rone: Difference between our use of pseudo-context and Query Expansion]
}

Although [\Rone] stated that our use of pseudo-context is very similar to a query expansion technique in information retrieval, we believe that there are fundamental differences between these two techniques.
According to our understanding, query expansion is a technique to expand or enrich the search query by using multiple techniques such as finding synonyms or semantically related words, fix spelling errors, re-writing the query with contextual information, etc.
However, our use of pseudo-context is more focused on constructing the input prompt as a dialogue format, which is impossible when we only have the utterances of a character.
The goal of using dialogue format prompt is to facilitate the in-context learning of the language model to generate a response that exhibits the style of character utterances, which have fundamentally different objective compared to query expansion.
Moreover, compared to the query expansion method that directly modifies or expands user query, our use of pseudo-contexts are for constructing pairs for statically given character utterances.
% Even if we interpret our method in a query expansion perspective which modifies the input to the language model using character utterances, comparison with the 'Only Utterances' baseline and PDP methods demonstrates that our new method of modifying the input prompt with the use of pseudo-contexts are much more effective than naively using only utterances.

\noindent \textbf{
[\Rone: Model might be re-synthesizing from the Pre-traning web data]
}

We agree that there might be a chance that the model has acquired knowledge about the character with the pre-training web data.
To investigate whether the model is blindly taking advantage of the pre-training dataset, we experimented with mimicking a new imaginary character that does not appear in the pre-training dataset nor the HLA-Chat dataset.
The result of this experiment was included in the Appendix of the previous version of the paper (Appendix H, "Mimicking a New Character" and Figure 4).
As shown in the example of a multi-turn conversation with an imaginary character (Pie the Duck), PDP successfully captures the character's unique language habits and produces identifiable responses while maintaining a dialog coherency.

\noindent \textbf{[\Rtwo, \Rfour: Model may copies the keyword/phrases in the character utterances]}

As the reviewer [\Rtwo] suggested, we provide the $n$-gram overlap for analyzing how the model copies the keyword/phrases from the references.
Appendix D.1 shows the result indicating that our method actively utilize the lexical phrases appearing in the character utterances.
This appearance will help people realize a better individualization of the specific character, nonetheless we also agree the concerns that the model may not capture inherent characteristics of the character.
However, addressing inherent characteristics is much more challenging since it is extremely difficult to define inherent characteristics of the character from a few utterances.
We think addressing inherent characteristics of characters will be intriguing future directions for our research.

\noindent \textbf{
[\Rthr: It is better to report the annotation consistency of human evaluation results]
}

Fleiss’ Kappas in our human evaluation are 0.112 and 0.067 for appropriateness and style strength, respectively, which are not high values. 
However, as Kulikov et al.\footnote{Importance of Search and Evaluation Strategies in Neural Dialogue Modeling, ACL 2019.} and Wong et al.\footnote{Wong et al., Cross-replication Reliability - An Empirical Approach to Interpreting Inter-rater Reliability, ACL 2021.} show on their paper, inter-rater reliability of annotation results using crowd-sourced annotators (such as our case, using Amazon Mechanical Turk) can be low since annotators show high cultural and training variances, especially when the task is subjective as our case.
Note that 99 annotators participated in our human evaluation.
Also, we limited the number of maximum annotations that a single annotator can be assigned to reduce the bias, which might have increased inter-rater diversity.
As we agree the reviewer's concern about evaluation reliability, similar to Kulikov et al. and Kim et al.\footnote{Will I Sound Like Me? Improving Persona Consistency in Dialogues through Pragmatic Self-Consciousness, EMNLP 2020.}, we included the Bayesian Calibrated version of human annotator scores to mitigate the noise from human annotations in the revised paper.

\noindent \textbf{
[\Rtwo: Comparison of the result of Gold Match with PDP \& other baselines]
}

The reviewer left good questions about our work.
First, [\Rtwo] asks why Gold Match shows worse performance in style strength than PDP. 
We believe that the context-response pairs in the HLA-Chat are not always the best pair for our situation.
Since HLA-Chat is originated from the scripts of the show, there might be some additional contexts outside of a single-turn dialogue (e.g., background of characters, events happened before the dialogue, audio-visual information, etc.)
We provide examples of a gold context-response pair from the script of BMO from The Adventure Time (context: "Yes! Take that, Princess Bubblegum!", response: "Jake Jr., I'm sorry for messing up your time travel.") and Burke from Grey's Anatomy (context: "I don't know, 75\%.", response: "Not good enough. He's my patient now. That okay with you, Dr. K?") which seems irrelevant without a background information about the TV show.
Without understanding the context behind the scripts, even gold context-response pair might seem irrelevant.
Therefore, directly using the context-response pairs in HLA-Chat as in Gold Match could adversely affect the quality of subsequent responses, in terms of style strength and coherency.
Conversely, our retriever is trained on a text-only dialogue without complex background information, so retriever is able to retrieve generally understandable pseudo-contexts.

Second, [\Rtwo] asks why Gold Match shows worse performance than baselines in terms of dialogue coherence.
For the case of human evaluation, Gold Match shows performance comparable to baselines.
However, Gold Match shows worse performance in terms of automated metrics, MaUdE.
We conjecture this phenomenon as follows.
MaUdE are tuned to work with texts in standard dialog style (e.g., DailyDialog, \textit{HLA-Chat}).
Thus, if generated responses strongly reflect character styles, then they are considered as out-of-domain cases for MaUdE so that there might be an unavoidable decrease in MaUdE scores.
This explanation is also described in Discussion part in Section 4.

As we agree that the performance comparison between PDP methods and the Gold Match is crucial for understanding the internal mechanism of our method, we will deeply investigate this topic in future work.

% Why gold match also shows worse performance than baselines in terms of dialogue coherence? These context-response pairs should have good coherency and will not affect the generation. 

\noindent \textbf{
[\Rtwo: A reason why Base-LM is better than other pre-trained LMs]
}

As [\Rtwo] mentioned, methods implemented using our pre-trained language model (Base-LM) show higher StyleProb values compared to other baseline methods.
The most significant difference between other pre-trained LMs and Base-LM is that Base-LM utilizes a large-scale dialogue dataset (Pushshift Reddit comment dataset) for the pre-training.
We believe that using dialogue data for training data leads LM to learn more about the inductive bias in the dialogue that the same speaker exhibits a similar language style, ultimately leading to better style strength performance in all methods.
We included this interpretation to the subsection in the Appendix F.1 in the revised version of the paper.

\noindent \textbf{
[\Rfour: Irrelevant utterances obtained by a retriever might impair the quality of the subsequent response]
}

We agree that the coherency between pseudo-context and character utterances largely affects the coherency of generated responses, as shown in the Table 1 (Static Match and Gold Match shows better coherency than Dynamic Match).
However, the relevance between pseudo context and character utterances does not necessarily negatively affect the style strength metrics, as shown in Random Match result.
We believe that investigating a method to retrieve contexts which are more relevant to character utterances (e.g. using more complex retrieval models) is an intriguing future direction for our research.

\noindent \textbf{
[\Rtwo: A reason for selecting BST for Context candidate]
}

We choose BST since it is one of the largest open-domain conversation dataset released in public, covering diverse topics and situations.
We include the explanation in our revised version of paper (in Section 2) about why we choose BST for context candidates.

\noindent \textbf {
[\Rfour: It would be better if an example of different characters in the same show is provided]
}

We provide more examples (Bart Simpson from The Simpsons and Dwight from The Office US) in Table 2 for revised version to present an example of the generated responses conditioned on different characters in the same show.
The examples show that distinct characters from the same show return different responses, which clarify that characters contribute to the difference.

\noindent \textbf{
[\Rthr: Is context candidate C single-turn, or multi-turn?]
}

We only utilize single-turn contexts as a context candidate, and we include the detail in the revised paper for clarification.

==> Tables/10_Utterance_Set.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{tabularx}{\linewidth}{l}
\toprule
\textbf{Spock} (from \textit{Star Trek}) \\
\midrule
\multicolumn{1}{l}{\begin{tabularx}{\linewidth}{X}
- Earth, Captain. We were on a general course in this direction when we were pulled in by the star. Apparently the breakaway threw us on in the same direction.\\
- Worry is a human emotion, Captain. I accept what has happened. The ship's hull seems to have a high density level or is cloaked against sensor probes. It is manned, but sensors cannot make out specifics.\\
- Recheck your equipment, Mister Scott. I'll scan for them on the planet's surface. Spock out.\\
- I submit, Mister Scott, if we do not get out, the shields would be extraneous. It would only prolong our wait for death by a short period of time.\\
- Our sensors are in a state of chaos, Captain. They became unreliable when we entered the Triangle.\\
- I have already begun investigation into that possibility.\\
- Captain, there are approximately one hundred of us engaged in this search, against one creature. The odds against you and I both being killed are 2,228.7 to 1.\\
- Spock here. Proceed, Mister Scott.\\
\end{tabularx}}\\
\toprule
\textbf{Sheldon Cooper} (from \textit{The Bigbang Theory}) \\
\midrule
\multicolumn{1}{l}{\begin{tabularx}{\linewidth}{X}
- I'm Dr. Sheldon Cooper, and welcome to the premiere episode of Sheldon Cooper Presents Fun with Flags. Over the next 52 weeks, you and I are going to explore the dynamic world of vexillology.\\
- Ah, normally I refrain from alcohol, but since my cerebral cortex is twiddling its proverbial thumbs, why not soak it in grape juice that's been predigested by a fungus?\\
- That's a semantically null sentence.\\
- Good morning and welcome to Science and Society. I'm Dr. Sheldon Cooper, BS, MS, MA, PhD, and ScD. OMG, right?\\
- Granted, my methods may have been somewhat unorthodox, but I think the end result will be a measurable enhancement of Penny's quality of life.\\
- Well, I've spent the last three hours in an online debate in the DC Comics Batman chatroom, and I need your help.\\
- I love strawberry Quik. It's my favourite pink fluid, narrowly beating out Pepto-Bismol.\\
- But I would like to remind you that in science, there's no such thing as failure. There once was a man who referred to his prediction of a cosmological constant as the single biggest blunder of his career. That man's name was, surprise, surprise, Albert Einstein.\\
\end{tabularx}}\\
\toprule
\textbf{Bart Simpson} (from \textit{The Simpsons}) \\
\midrule
\multicolumn{1}{l}{\begin{tabularx}{\linewidth}{X}
- Oh man, you girls ruin everything -- even vampires.\\
- We're Simpsons, Dad. We don't do good behavior.\\
- I'm sorry for all the trouble I've caused you, Krusty. But, you know, my mom says God never closes a door without opening a window.\\
- Come on, Lis. Let's go finish our soapbox racers.\\
- I didn't ruin Thanksgiving! She did... Buncha jerks... I always get blamed for everything...\\
- Mom, this gravy tastes better than God's sweat.\\
- Quick, Mom! Whip up a cake before Dad fires you!\\
- Hey, Dad, why don't we try the "Sprawl-Mart"?\\
\end{tabularx}}\\
\toprule
\textbf{Marge Simpson} (from \textit{The Simpsons}) \\
\midrule
\multicolumn{1}{l}{\begin{tabularx}{\linewidth}{X}
- You should've seen the faces of your children when they caught you stealing. Kids, get in here and show your father the faces!\\
- Aw, Homie, you'll always be my western hero.\\
- Isn't Bart sweet, Homer? He sings like a little angel.\\
- Bart! That hobo skeleton is not a toy!\\
- Homer, please!\\
- You're teaching Bart a terrible lesson of intolerance!\\
- Bart? Honey, I made you an extra-warm sweater you can wear while you're down in the well.\\
- Okay, Bart, you don't have to say it, but you do have to have a loving attitude. Be nice to your sister.\\
\end{tabularx}}\\
\bottomrule
\end{tabularx}
\caption{Utterance set used for describing the subset of characters used for our experiments.}
\label{tab:10-1_utterance_set}
\end{table*}

\begin{table*}[t]
\centering
\footnotesize
\begin{tabularx}{\linewidth}{l}
\toprule
\textbf{BMO} (from \textit{Adventure Time with Finn \& Jake}) \\
\midrule
\multicolumn{1}{l}{\begin{tabularx}{\linewidth}{X}
- Jake Jr., I'm sorry for messing up your time travel.\\
- Ronnie the mouse stole it, but Lorraine chicken set him up to kill Bebe, but the flatfoot busted Ronnie, and Lorraine skedaddled with the loot, but BMO solved the case!\\
- They're too strong! Use the combo move, Finn! The combo-\\
- Okay. Please take me to get fixed. I need- need- need- need to get new core system drivers installed. We can get them at the MO Factory in the Bad Lands, where I was born.\\
- Yippie ki-yi-yay!\\
- I'm gonna go wash this shmutz off my grabbers.\\
- Sorry, lady, forgetting ain't in my job description. Ha ha ha!\\
- If anyone tries to hurt Finn, I will kill them.\\
\end{tabularx}}\\
\toprule
\textbf{Rachel} (from \textit{Friends}) \\% & \textbf{Sheldon Cooper} (from \textit{The Bigbang Theory})\\
\midrule
\multicolumn{1}{l}{\begin{tabularx}{\linewidth}{X}
- Oh my God, Phoebe, this is impossible! We can't do this by Friday! We have to find a place. We have to invite people! We have to get food! There's just too much to do! It's impossible! We can't do it! We cannot do it! We cannot do it! \\
- Jo-Joey, look honey we-we need to talk okay? Umm, I kinda got the feeling from her today that uh, she's not lookin' for a serious relationship.\\
- Hey, come on! I had this friend from college and I made the stupid mistake of telling Joey that one time…she and I y'know…kissed a little bit.\\
- Ooh, I miss dating. Gettin' all dressed up and going to a fancy restaurant. I'm not gonna be able to do that for so long, and it's so much fun! I mean not that sitting at home worrying about giving birth to a sixteen pound baby is not fun.\\
- Oh, y'know, would you just for once, not remember every…little…thing!!\\
- Yeah I don't think dressing provocatively is going to help me here! Oh my god just please take her.\\
- Okay. It's okay. We're gonna be okay. Y'know what? It's okay. I'm gonna, I'm gonna, I'm gonna boil some water and just rip up some sheets!\\
- Oh, I mean she's gonna be at the wedding waiting for him and people will be whispering, "Oh that poor girl." Y'know? Then she'll have to come back here and live all alone.\\
\end{tabularx}}\\
\toprule
\textbf{Michael} (from \textit{The Office US}) \\% & \textbf{Sheldon Cooper} (from \textit{The Bigbang Theory})\\
\midrule
\multicolumn{1}{l}{\begin{tabularx}{\linewidth}{X}
- Dwight, oh ho, Dwight, Dwight, my loyal compadre. You and I are hangin' tonight. The two of us. We are celebrating our freedom and our manhood. You know what? Why don't we watch that show that you've been wanting to watch, that stupid Battleship Galaxy.\\
- No, no, no. I am not dating Jan. She was very clear about that. Just two like souls having a romantic time in the most romantic place on earth. Got enough, weirdo?\\
- I'm not firing him. I'm not, I need you to act like I am firing him. Just, what I'm going to do, is I'm going to pretend that I am firing him, and I need you to act like I am firing him. Do you get that? Do you get it? I'm teaching him a lesson. He needs to learn humility, alright? That's all I'm, okay, here he comes. Let's just... play act.\\
- EHHHHNT. Game over. Offer revoked. Dwight. I'm sorry, but you reach out and you try to be a nice guy, and help out a friend, and this is what happens. This is what I get. Oh god. I'm ... Ok.\\
- All right, let's not get hung up on the furnace. This just... it's the sales... I see the sales department down there. They're in the engine room, and they are shoveling coal into the furnace, right? I mean, who saw the movie Titanic? They were very important in the movie Titanic. Who saw it? Show of hands!\\
- Oh, cool. Cool. And maybe you could attend tonight and then you could stay over at my house for the night. Awkward. That's... You know what. Brenda, could Jan and I have a moment alone?\\
- No problem. The guys are having a little shindig of their own in the warehouse. From 2:30 to 3:15. It is the only time that Bob was available. Sort of a guy's night out. A G-N-O if you will. A Gah-No. Actually, it's more of a guy's afternoon in. A G-A-I. A gay. Not- not- it's uh, not gay, it's just a, it's a bridal shower for guys. A guy shower. An hour long shower with guys.\\
- Just follow my lead. Don't pimp me, all right? Come in. So, uh, Corporate just said that I don't want to...\\
\end{tabularx}}\\
\bottomrule
\end{tabularx}
\caption{Utterance set used for describing the subset of characters used for our experiments.}
\label{tab:10-2_utterance_set}
\end{table*}

\begin{table*}[t]
\centering
\footnotesize
\begin{tabularx}{\linewidth}{l}
\toprule
\textbf{Burke} (from \textit{Gray's Anatomy}) \\
\midrule
\multicolumn{1}{l}{\begin{tabularx}{\linewidth}{X}
- Dr. Yang. I don't need you for this. This is a known complication of the surgery. It happens. It happens. Restart bypass.\\
- No, I can fix her heart while it's still beating. Push 40 milligrams of abizonole.\\
- That's not for you to decide Dr. Grey. He asked you for something. You told him you would do it. If you don't, that doesn't make you noble. It makes you a liar.\\
- Christina I can't walk away from this surgery. If I do this man will die. So tremor or no tremor, I have to try. But you..\\
- I want to know when you stopped thinking of me as your number one. Richard, I do more in this hospital than any other surgeon.\\
- We're finished here, Karev. You're off this case.\\
- I am the best surgeon at Grace with the lowest mortality rate, you can't just bring some guy in from -\\
- Not good enough. He's my patient now. That okay with you, Dr. K?\\
\end{tabularx}}\\
\toprule
\textbf{Barney} (from \textit{How I Met your Mother}) \\% & \textbf{Sheldon Cooper} (from \textit{The Bigbang Theory})\\
\midrule
\multicolumn{1}{l}{\begin{tabularx}{\linewidth}{X}
- Unfair? I wouldn't let you take care of the imaginary kids I make up to score with single moms. That's it Ted, we're going home. Ted? Ted, you okay?\\
- Yes! Yes! We're back. We are back. And Ted, my boy, it's going to be legend... Wait for it...\\
- Robin, girls are like cartons of milk. Each one has a hotness expiration date, and you've hit yours. I'm not saying the occasional guy won't still open the fridge, pick you up, give a sniff, shrug and take a sip anyway But it's all downhill from here.\\
- Oh, Robin, my simple friend from the untamed north, let me tell you about a little thing I like to call mind over body. You see, whenever I start feeling sick, I just stop being sick and be awesome instead. True story. Yeah, in two minutes, I'm going to pound a sixer of Red Bull, hop in a cab, play a couple of hours of laser tag, maybe get a spray-on tan. It's gonna be legen... Wait for it...\\
- No, no, no... we are not laughing about this, Ted. This is not going to be some funny story that we'll be telling in a couple months. It's not gonna be like, "Hey, remember that time when you were grinding with... NO! And you know why? Because, italics, this night did not happen. And you promise me that you will never, ever, ever tell another soul what transpired here tonight. You promise. Promise\\
- You're right, I do deserve that. That's all I came here to say. You know what? I don't care who knows about it. Excuse me. Excuse me. I, Ted Mosby, am a jerk to women. Tell your sisters. Tell your daughters to stay away! Ted-Mosby-Is-A-Jerk-dot-com.\\
- Please, vacation romances have an expiration date. Gael's got a "Best if banged by" sticker on him. Once your romance starts to stink, you'll dump his ass down the drain like sour milk and go back to being "Unevolved Robin", the one we actually like. Back me up here, Ted.\\
- I need alcohol. I'm not gonna do that stuff with Robin.Look at that. Berry cocktail, conditioner meninges. I dream, these drinks could make a girl smarter. What hell Ted brought us?\\
\end{tabularx}}\\
\toprule
\textbf{Dwight} (from \textit{The Office US}) \\% & \textbf{Sheldon Cooper} (from \textit{The Bigbang Theory})\\
\midrule
\multicolumn{1}{l}{\begin{tabularx}{\linewidth}{X}
- Can I have my neck pillow back? Michael! Can I have my neck pillow back?\\
- How bout this. I don't tell Michael and in exchange you owe me one great big giant favor. Redeemable by me at a time and place of my choosing.
- Michael, please. Stop it now. You're embarrassing yourself.\\
- Thank you Michael. I just want to say, to the few of you who will remain under my employ, that I intend to lead you into the black! With ferocity!\\
- Black Bears can smell a salami at five miles Michael, what are you thinking?! And they run faster than a horse, so if you were thinking about outrunning one on a horse I would try a cheetah. You, in tight pants, Michael, are a salami to a Black Bear. Do you understand?\\
- Michael, I have so much to learn from you.\\
- Don't let him in! He's a traitor! Michael!\\
- Dammit. I am no closer to taking Jim down. What a waste of a day. I could of grown poisoned mushrooms that would have been this high by now.\\
\end{tabularx}}\\
\bottomrule
\end{tabularx}
\caption{Utterance set used for describing the subset of characters used for our experiments.}
\label{tab:10-3_utterance_set}
\end{table*}


==> Tables/13_Arb_Style_Prompt.tex <==
\begin{table*}[t]
\centering
\footnotesize
\begin{tabular}{l}
\toprule
\textbf{Template} \\
\midrule
\multicolumn{1}{l}{\begin{tabular}[l]{l}
\texttt{Following are past utterances by \{\{ character\_name \}\}:}\\
\texttt{\{\{ u1 \}\}} \\
\texttt{\{\{ u2 \}\}} \\
\texttt{Rewrite ``\{\{ Base-LM Response \}\}'' in \{\{ character\_name \}\}’s style:}\end{tabular}} \\
\midrule
\textbf{Example Prompt} \\
\midrule
\multicolumn{1}{l}{\begin{tabular}[l]{l}
Following are past utterances by Marge Simpson from The Simpsons:\\
Marge Simpson from The Simpsons: Aw, Homie, you'll always be my western hero.\\
Marge Simpson from The Simpsons: Isn't Bart sweet, Homer? \\
Rewrite ``I have to go back on December 8th.'' in Marge Simpson from The Simpsons's style: \end{tabular}} \\
\bottomrule
\end{tabular}
\caption{Prompt template and example prompt for Base-LM + Arb Style.}
\label{tab:arb_style_prompt}
\end{table*}


==> Tables/99_Cherry_Picked.tex <==
\begin{table}[]
\centering
\footnotesize
\setlength
\tabcolsep{2.5pt}
\begin{tabular}{l}
\toprule
\multicolumn{1}{l}{\begin{tabular}[l]{l}\textbf{Input}: We'll pick you up at your place at noon. \\Be there or be square!\end{tabular}} \\ 
\midrule
 \multicolumn{1}{l}{\begin{tabular}[l]{l}\textbf{Marge Simpson from the Simpsons}: Homer, you are\\
 my rock! I'm counting on you!\end{tabular}} \\

\cmidrule(lr){1-1}
\multicolumn{1}{l}{\begin{tabular}[l]{l}\textbf{Michael from The Office US}: I will be there. \\
I will be there! I will be there, all right? \\
So, just... be ready. Don't be late. You know, I'm sorry.\end{tabular}} \\

\cmidrule(lr){1-1}
\multicolumn{1}{l}{\begin{tabular}[l]{l}\textbf{Rachel from Friends}: Oh my god, Phoebe, I just-\end{tabular}} \\

\cmidrule(lr){1-1}
\multicolumn{1}{l}{\begin{tabular}[l]{l}\textbf{Sheldon from The Bigbang Theory}: Okay, well, \\
see you at noon! Goodbye.\end{tabular}} \\

\cmidrule(lr){1-1}
\multicolumn{1}{l}{\begin{tabular}[l]{l}\textbf{Spock from Star Trek}: Aye, Mister Scott. I'll be there.\end{tabular}} \\
\bottomrule
\end{tabular}
\caption{More examples for responses generated by using Dynamic Match for each character.}
\label{tab:7_cherry_pick}
\end{table}


==> Tables/99_Main_Results_With_Std_Human.tex <==
\begin{table*}[t]
\centering
\footnotesize\setlength\tabcolsep{5pt}
\begin{tabular}{clccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}[2]{*}{\begin{tabular}[c]{c}Method \\Type\end{tabular}}} & \multicolumn{1}{c}{\multirow{2}[2]{*}{Methods}} & \multicolumn{3}{c}{Human Evaluation} & \multicolumn{2}{c}{Automatic Evaluation} \\ \cmidrule(lr){3-5}  \cmidrule(lr){6-7}
& & \multicolumn{1}{c}{Style.} & \multicolumn{1}{c}{Appr.}  & \multicolumn{1}{c}{Sum}  & \multicolumn{1}{c}{StyleProb} & \multicolumn{1}{c}{MaUdE} \\
\midrule
\multirow{5}{*}{\textbf{Baselines}}
& Base-LM + TextSETTR& 1.155 $\pm$ 0.051 & \textbf{1.317} $\pm$ 0.050 & 2.472&  0.1045 $\pm$ 0.0013 & 0.8435 $\pm$ 0.0019\\
& Base-LM + ArbStyle & 1.188 $\pm$ 0.053 & 1.219 $\pm$ 0.049 & 2.407& 0.1921 $\pm$ 0.0023& 0.7701 $\pm$ 0.0026\\
& Zero-shot Prompt& 1.172 $\pm$ 0.051 & 1.236 $\pm$ 0.049 & 2.408& 0.1432 $\pm$ 0.0018& \underline{\textbf{0.8857}} $\pm$ 0.0016\\
& GCC& 1.193 $\pm$ 0.051& 1.256 $\pm$ 0.048& 2.449& 0.2391 $\pm$ 0.0024& 0.8835 $\pm$ 0.0017\\
& Only Utterances& 1.200 $\pm$ 0.052& 1.263 $\pm$ 0.049& 2.463& 0.2098 $\pm$ 0.0023& 0.8887 $\pm$ 0.0016\\
\midrule
\multirow{3}{*}{\textbf{Ours}}
& Dynamic Match& \underline{\textbf{1.331}} $\pm$ 0.049& 1.203 $\pm$ 0.051& \textbf{2.534}&  \underline{\textbf{0.4789}} $\pm$ 0.0032& 0.8299 $\pm$ 0.0019\\
& Static Match& 1.277 $\pm$ 0.052 & 1.229 $\pm$ 0.052& 2.506& 0.4192 $\pm$ 0.0031& 0.8467 $\pm$ 0.0018\\
& Random Match& 1.297 $\pm$ 0.050& 1.195 $\pm$ 0.053& 2.492& 0.4774 $\pm$ 0.0032& 0.8358 $\pm$ 0.0019\\
\midrule
\midrule
\multirow{2}{*}{\textbf{Oracle}}
& Full-shot Fine-tuning& 1.260 $\pm$ 0.051& \underline{1.329} $\pm$ 0.049& \underline{2.589}& 0.2880 $\pm$ 0.0027& 0.8793 $\pm$ 0.0028\\
& Gold Match &1.287 $\pm$ 0.050& 1.245 $\pm$ 0.051& 2.532&  0.4575 $\pm$ 0.0032 & 0.8350 $\pm$ 0.0019\\
\bottomrule
\end{tabular}
\caption{Evaluation results of style strength and appropriateness.
Underlined score indicates the best result among all methods, and bolded score indicates the best result among the baselines and our methods for each metric.}
\vspace*{-2mm}
\label{tab:main_result_appendix}
\end{table*}




































